Extraction of Complex DNN Models: Real Threat or Boogeyman?

Recently, machine learning (ML) has introduced advanced solutions to many domains. Since ML models provide business advantage to model owners, protecting intellectual property of ML models has emerged as an important consideration. Confidentiality of ML models can be protected by exposing them to clients only via prediction APIs. However, model extraction attacks can steal the functionality of ML models using the information leaked to clients through the results returned via the API. In this work, we question whether model extraction is a serious threat to complex, real-life ML models. We evaluate the current state-of-the-art model extraction attack (Knockoff nets) against complex models. We reproduce and confirm the results in the original paper. But we also show that the performance of this attack can be limited by several factors, including ML model architecture and the granularity of API response. Furthermore, we introduce a defense based on distinguishing queries used for Knockoff nets from benign queries. Despite the limitations of the Knockoff nets, we show that a more realistic adversary can effectively steal complex ML models and evade known defenses.

==> discussion.tex <==
%auto-ignore
\section{Discussion}
\label{sec:discussion}

In this work, we extended the evaluation of the KnockOff attack and assessed it in several new scenarios.
We showed that its performance depends on the quality of the transfer set used to carry out the attack.
Relying solely on a large set of unlabeled data is not sufficient to achieve high accuracy on datasets with complex features.
What is more, resulting surrogate model has imbalanced per-class accuracies which limits its usage.
We demonstrated that choice of generic hyperparameters (e.g. batch size or number of epochs) yields subpar performance that could be further improved.
In practice, this might be infeasible due to lack of high quality ground-truth test data.
However, adversary with such an enhanced training strategy could reach even higher accuracy than originally reported.
Furthermore, we showcased that mismatch between architectures of the victim and surrogate models further hinders the efficacy of model extraction.
While similar conclusion was reached in prior work~\cite{juuti2019prada}, it was limited to model extraction attacks using synthetic data.

On the other hand, we observed that the larger the overlap between \adv's and victim's distribution, the less plausible the detection is.
Publicly available datasets designed for ML research as well as vast databases accessible through search engines and from data vendors (e.g. Quandl~\cite{quandl}, DataSift~\cite{datasift}, Axciom~\cite{axciom}) allow \adv to obtain substantial amount of data from any domain.
Therefore, one can argue that making assumptions about \adv's access to natural data (or lack of thereof) is not realistic.
This corresponds to the most capable, and yet plausible, adversary model - one in which \adv has approximate knowledge about victim's distribution and access to a large number of unlabeled samples.
In such scenario, \adv's querying samples are not going to differ from an average benign \client, rendering detection techniques ineffective,

As a result, it is questionable whether offering ML models via open prediction APIs is safe.
Even if model extraction can be detected through stateful analysis, highly distributed Sybil attacks are unlikely to be detected.
In theory, vendors could charge their customers upfront for a significant number of queries (over 100k), making Sybil attacks cost-ineffective.
However, this reduces utility for benign users and restricts the access only to those who can afford the down payment.
Alternatively, usage of ML models could be restricted to internal processes and channels that are not directly exposed to the user (e.g. encrypted communication between a smartphone and a server) or even to trusted hardware such as secure enclaves (e.g. Intel SGX~\cite{mckeen2016sgx}).
Nevertheless, there is no guarantee that IP associated with the ML model can be protected.

